Low Sample Complexity Participatory Budgeting

We study low sample complexity mechanisms in participatory budgeting (PB), where each voter votes for a preferred allocation of funds to various projects, subject to project costs and total spending constraints. We analyze the distortion that PB mechanisms introduce relative to the minimum-social-cost outcome in expectation. The Random Dictator mechanism for this problem obtains a distortion of 2. In a special case where every voter votes for exactly one project, [Fain et al '17] obtain a distortion of 4/3 We show that when PB outcomes are determined as any convex combination of the votes of two voters, the distortion is 2. When three uniformly randomly sampled votes are used, we give a PB mechanism that obtains a distortion of at most 1.66, thus breaking the barrier of 2 with the smallest possible sample complexity. We give a randomized Nash bargaining scheme where two uniformly randomly chosen voters bargain with the disagreement point as the vote of a voter chosen uniformly at random. This mechanism has a distortion of at most 1.66. We provide a lower bound of 1.38 for the distortion of this scheme. Further, we show that PB mechanisms that output a median of the votes of three voters chosen uniformly at random have a distortion of at most 1.80.

==> intro.tex <==
\section{Introduction}
More than 1500 cities around the globe have begun adopting {\it Participatory Budgeting} (PB) \cite{wainwright2003,ganuza2012}, 
a process through which residents can vote
directly on a city government's use of public funds.  Citizens might, for example,
vote directly on how to allocate a budget of reserved funds between projects like
street repairs or library renovations.  PB has been shown to promote
government transparency, citizen engagement, and good governance \cite{wampler2007}.

PB implementations have used various mechanisms to elicit preferred budgets from citizens 
\cite{brams2002voting,arrow2010handbook,goel2019knapsack,benade2021preference}. %, yet no matter the mechanism,
Policymakers must then transform a list of votes on a budget into a real-world allocation of funds.
Furthermore, even though there may be an ``optimal'' allocation (under natural notions
of social welfare),
this allocation may be intractable to compute \cite{jain2020,peters2020proportional} or difficult to reliably estimate if turnout is low \cite{ewens2019organizational}.
Our topic of study in this work is the {\it distortion} that PB mechanisms introduce
between the theoretically ``optimal'' allocation and the output by the mechanism.

%Participatory budgeting (PB) is a process in which citizens vote on the public budget. For example, residents of a city may vote on how to spend a million dollars of the city's funds on projects such as renovating the library or improving the streets. PB first started in the 1980s in Brazil \cite{wainwright2003} and is gaining popularity, with more than 1,500 cities worldwide already adopting PB \cite{ganuza2012}. %PB has been shown to promote transparency, citizen involvement, and good governance \cite{wampler2007}.
%
%Several voting methods have been used in PB, such as %\emph{K-approval voting}, in which voters approve up to $K$ projects from the list of all projects,
%\emph{approval voting} \cite{brams2002voting,arrow2010handbook}, in which voters select any number of projects that they like, and \emph{knapsack voting} \cite{goel2019knapsack}, in which voters select as many projects as they like, subject to the budget constraint. Major challenges in PB include low voter turnaround \cite{ewens2019organizational}, and the design of ballots accounting for substitute and complementary projects \cite{fairstein2021proportional, jain2020, jain2021partition}.


{
In particular, we focus on a process known as {\it sequential deliberation} \cite{fain2017,fishkin2018democracy},
a mechanism for collective decision-making % (in contexts where citizens can debate directly)
 that we \remove{adapt}{\color{red}  use as the first pre-processing step} %into a mechanism 
 for PB. {\color{red} Typically in most PB instances, there involves a deliberation step where the projects are discussed and bundled accordingly as described in \cite{deliberation_participatory_budegting,gilman_deliberation,https://doi.org/10.1002/pad.1853}.}
In each round of sequential deliberation,
two randomly-selected voters debate to decide on a compromise, which becomes the ``disagreement point''
for the next round.  If the voters in a round fail to reach a compromise, their choice defaults to the disagreement
point of the previous round; as such,
the disagreement point, in essence, captures an aggregate preference of the deliberators of previous rounds.

}
%
%To extend this process to PB (where a ``deliberation'' must be between static votes, not living voters),
%we propose and analyze several \XXX{several? one? two?} classes of ``bargaining'' mechanisms for algorithmically aggregating two random budget votes
%and a disagreement point into a new disagreement point (and let the disagreement point of the first round be a third, random vote).
%
%On another but related note, public deliberation has been gaining popularity as a democratic process for collective decision-making \cite{fishkin2018democracy}. %It has several good properties, including the potential for coming up with more innovative solutions, and enabling people to understand each others' point of views \cite{fishkin1991democracy}.
%Sequential deliberation has been proposed as a method for implementing deliberation among agents \cite{fain2017} in which randomly chosen agents deliberate in pairs in rounds, and the outcome of the previous round is the disagreement point for the new round. (The disagreement point of a bargaining process is the outcome if no agreement is reached by the parties). The disagreement point, in essence, distills the preferences of all the agents who participated in the previous rounds. In this paper, we propose a sequential deliberation-based mechanism for PB. 
%
Our theoretical guarantees are for the outcome of one round of deliberation. This mechanism takes only three samples of the voters (one for the disagreement point and two for deliberation) and is therefore also interesting for the goal of minimizing the sample-complexity of the mechanism.\footnote{See also Fain et al. \cite{fain2019} for another PB mechanism with a sample-complexity of 3.}% An important part of our sequential deliberation scheme is that the agents are chosen at each round without the knowledge of the precise bargaining scheme adopted in each round of deliberation, hence it may be adopted to a variety of settings.}
 
\XXX{Low complexity mechanisms was well understood for median spaces in SD paper but not with budget constraints and L1 setting.}

\XXX{show that random referee will not work with PB and will get distortion 2; show by the start example}

{\color{red} Sequential deliberation in this setup}\remove{The use of sequential deliberation in PB} has some properties that are especially interesting to policymakers. For example, we will demonstrate with simulations in \S\ref{sec:exp} that sequential deliberation can very rapidly converge to a solution that has a limited "distortion". This means that with a few rounds of deliberations, %each only requiring participation from a very small sample,
we can get an estimate of what budgetary region the result of a vote could lie in. This could be particularly important in scenarios where turnout is low, or a PB ballot must be simplified before deployment \cite{aitamurto2015five}.

There are also some intrinsic advantages to using sequential deliberation to collect budgeting preferences. For example, the bargaining process will encourage voters to exchange ideas and opinions in a short, focused period of time that allows the organizer to collect the arguments in connection with certain disagreements in the budget space efficiently. Any deliberative process where different voters constructively interact with other voters would expose voters to opinions from other voters, which has potential benefits to the democratic process \cite{christ2019intergroup}. 

One important feature of sequential deliberation is that the outcome
is guaranteed to be the preference of a pair of individuals;
this means that the outcome will always account for complex interactions between different projects (such as substitutability and complementarity \cite{jain2020, jain2021partition}). We define these terms precisely and show that our proposed mechanism naturally accommodates these complex preferences in Appendix \S \ref{sec:TD_project_interaction}. 

%Some recent works have proposed randomized voting schemes. In some voting schemes, voters report a pairwise comparison between randomly chosen budget proposals \cite{fain2019}, voters may report a set of projects with utility higher than a randomly set threshold \cite{bhaskar2018truthful}. Our proposed sequential deliberation-based method is also a randomized voting mechanism. %It will arguably be less costly to implement than standard PB elections since much fewer voters need to participate and deliberation has been shown to result in more innovate solutions to societal issues \cite{fishkin1991democracy}.

%Two types of PB elections have been studied: those designing the entire budget and those deciding the allocation of funds to a fixed set of projects under a given budget constraint. We study the latter in this work.

\remove{
\subsection{Project Interactions in PB}
Most theoretical work on PB assumes that different projects can be implemented independently. However, in many practical situations, this assumption is not valid. Several projects can be substitutes for each other. As an example, consider the two projects of building a park each on road A and road B. If the two roads are close to each other, the residents of the area would see the two projects as substitutes for each other and pick one arbitrarily in their vote. We define a group $S$ of projects to be \emph{perfect substitutes} if no voter wants more than one project in $S$ to be funded. The utility that voters can derive from group $S$ is the maximum funding of a project in $S$. %For example, if two companies are paid $0.2$ and $0.5$ to do the same work, only $0.5$ will be used, and $0.2$ is wasted. 
In another scenario, projects can be complements of each other. For example, buying new computer hardware and software may be seen as complementary projects by the voters. We define a group of projects $R$ to be perfect complements if the utility that voters can derive from each project in $R$ is the minimum funding of any project in $R$. For example, if the software and hardware projects are funded $0.2$ and $0.5,$ they can only use $0.2$ each, and the excess funding of $0.3$ for the hardware project is wasted. These are special cases of submodular and supermodular utility functions for substitute and complement projects, respectively. Further, we define a group of projects to be contradictions if it is physically impossible to implement more than one of them. %As noted by Jain, Talmon, and Bulteau in \cite{jain2021partition}, the utility of agents may be given by a submodular function over the set of \emph{substitute} projects, and by a supermodular function over the set of \emph{complementary} projects. 
 %Such project interactions may sometimes be unknown to the PB designers or may be difficult to account for in the ballot.
} 

%Jain, Sornat, and Talmon \cite{jain2020} introduce a model in which the project interactions are specified in the ballot and the voters do approval voting. They provide algorithms for vote aggregation aimed at utility maximization under different functions of  

{\raggedleft\textbf{Our Contributions}}

%In this paper, we study two settings for dealing with project interactions in PB, \textit{sequential deliberation}.\remove{ and a \textit{menu-based ballot design}.} \edit{While these two approaches have different models and assumptions, they both provide useful insight into how PB could generalize beyond non-interactive projects.} In the former, 

%Voters bargain in pairs in rounds, with the outcome of the previous round being the disagreement point for the new round. (The disagreement point of a bargaining process is the outcome if no agreement is reached by the parties.)
%
%We show that this simple mechanism has some desirable properties. One is that it has a distortion\footnote{Distortion measures how far the outcome of a voting mechanism is from the social-welfare-maximizing outcome in the worst case; it is defined more formally in \S~\ref{sec:distortion_defn}.} of at most 1.66, which is a significant improvement over the \emph{random dictator} mechanism which has a distortion of 2. Another property is the ability to handle perfect complementary and perfect substitute project interactions without explicit input from the PB designer. 
%Since voters are residents who would benefit from implementing the projects on the ballot, they implicitly know the project interactions. 
%This ensures that the outcome of the deliberations will not waste money by funding only one project in a perfect complementary group or funding multiple projects in a \edit{perfect} substitute group, which can happen in other voting methods. In this framework, we make the stylized assumption that all voters agree on the project interactions, \edit{and these interactions are not transparent to the ballot designers or to the voting mechanism.} %This is a reasonable assumption in most practical scenarios. 

%We adopt the \emph{overlap utility} model, which is the same as the $l_1$ distance of two budgets~\cite{goel2019knapsack,freeman2021truthful}. In this model, each voter has a preferred budget, and the utility that they gain from an allocation equals how much it has in common with their preferred budget.
%We show that if the bargaining process satisfies the axioms of \emph{Nash bargaining} \cite{binmore1986nash},
%then the total overlap utility of voters involved in the deliberation and of the disagreement point, is maximized. 


 Following Anshelevich et al. \cite{anshelevich2017randomized}, we study the \textit{distortion} of a mechanism, which measures the \emph{social cost} of the output of the mechanism relative to a social-cost-minimizing outcome. Here the cost function is the $\ell_1$ distance between budget allocations, {\color{red} a similar metric adopted in \cite{FREEMAN2021105234}.} We show that natural mechanisms in which two uniformly randomly chosen agents bargain \emph{without} considering a disagreement point cannot have a distortion less than $2$. 
In contrast, we show that using a disagreement point
enables mechanisms that are guaranteed to have distortion substantially below $2$.
%Therefore we propose mechanisms in which two agents deliberate with a disagreement point generated from the previous round of deliberations.
%
Specifically, we show first that all bargaining mechanisms in a class of \emph{median bargaining schemes} achieve distortion
of at most $1.80$ after just one round of deliberation. Furthermore, we also give a \emph{randomized Nash bargaining scheme}
that achieves distortion of at most $1.66$ after one round.

The main technical tool we use is the analysis of \emph{pessimistic distortion} (PD) first proposed by Fain et al. \cite{fain2019}. PD is a form of distortion where the counterfactual is allowed to choose a separate outcome for every small subset of the voters (of a fixed size), thereby attaining a lower social cost than the true `optimal'. We use the PD as an upper bound on the distortion of our proposed mechanism. We then reduce the problem of computing the PD into a set of linear {and bilinear} programs. \remove{for \color{red} $\mathcal{M}$ and a set of bilinear programs for $\mathfrak{n}_{\text{rand}}.$ -- undefined terms.} The problem has a complex combinatorial structure due to the nuances of Nash bargaining. However, we are able to exploit symmetries of the problem to significantly reduce the number of optimization programs that are required to be solved. %We provide the code for solving these problems on GitHub\footnote{\textcolor{red}{PUT LINK TO CODE}}. 


%\edit{This means that for all possible instances of PB, the allocation that results from sequential deliberation has a total \emph{disutility} less than $1.66$ times that of the social welfare-maximizing allocation in expectation, where the expectation is over the randomness in the bargaining process.}

%This result is interesting because any voting mechanism constrained to choose outcomes from the voters' preferred budgets has an expected distortion at least 2.
%\edit{In the sequential deliberation approach, the bound on the distortion assuming there are no project interactions is also valid if there are project interactions.} Interestingly, this is the first voting mechanism that provably has distortion below $2$ for PB with interdependent projects; any voting mechanism constrained to choose outcomes from the voters’ preferred budgets has distortion at least $2$ (Lemma~\ref{dist2}). 

We also propose a sequential deliberation mechanism, an extension to the bargaining scheme by setting the disagreement point for each round as the outcome of the previous round in Appendix \ref{sec:exp} and also evaluate the proposed mechanism empirically using data from real participatory budgeting elections. %\edit{These empirical results are without project interactions.} 
We observe that the expected distortion after two rounds of sequential deliberation is less than $1.30$ for all four PB elections we study. Further, the variance of the allocations to projects converges to a small value after just three rounds of deliberation. %This validates our approach on real-world datasets. % what elections? % should we include fast convergence here?

\remove{
\edit{When the project interactions are given explicitly by the PB designer, we study a menu-based ballot design. Such ballot designs are growing in popularity in PB and gaining a theoretical insight into them is important. For example, the 2020 city budget consultation in Long Beach conducted on the Stanford City Budgeting Platform\footnote{\url{https://budget.pbstanford.org/longBeach2020}} had a menu-based ballot with some complex project interactions. We study a simplified model of such a ballot. %In this setting, we relax the assumption that all voters agree on the project interactions. 
%We further relax the assumption that projects in a group of substitutes are perfect substitutes. 
%This model can work with both fractional and non-fractional funding of projects. 
 In our model, }the PB designer divides the projects into groups such that the voters' utilities are additively separable over the different groups. Groups correspond to contradictory, substitute, or independent projects. Independent projects correspond to groups of size $1$.  %We consider a natural extension of the overlap utility model. 
For preference aggregation, the voters do approval voting within a group and distribute money across groups as in knapsack voting. 
%with the constraint that the cost of approved projects in a group is at least as much as the money allocated to the group by the voter. 
This ballot design makes voting cognitively easier than knapsack voting, where voters must allocate money to each project separately. %At the same time, it elicits more information regarding preferences than approval or K-approval voting. 
In many practical situations, some voters only care about broad issues such as healthcare, security, education, etc. In our proposed ballot, the project groups may correspond to these broad issues, with individual projects listed within the groups. Voters would spend more cognitive effort in deciding how to allocate funds to the broad issues; and then approve their favored projects in the groups, usually with less cognitive load.

 \edit{ %If voters think that the projects in a group are substitutes or contradictions, they would allocate one unit of funds, and approve all the acceptable projects in the group. If voters wish to fund $2$ projects from a group but find $5$ options acceptable, they can allocate two unit of funds, and approve the $5$ acceptable projects in the group. 
%It is noteworthy that this is the first ballot design which can handle both project substitutions and contradictions by the same preference elicitation and aggregation method. 
 Our proposed ballot enables the handling of project interactions where projects are either substitutes or contradictions, and is the first ballot design capable of doing so.} For unit cost projects, we show that for social welfare-maximizing preference aggregation, our method is strategy-proof when at most one project from a group can be funded.  %If voters think that the projects are complementary, they would fund the project group for as many units as they think should be funded, and approve the projects they think should be funded together. 
%For the menu-based ballot, we consider both fractional and non-fractional allocations. 
We show that under non-fractional allocations, maximizing social welfare is NP-hard by reduction from the maximum set cover problem. We then provide a dynamic programming-based %fixed parameter tractable (FPT) 
algorithm for maximizing social welfare%, parameterized by the maximum size of a group
.}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
{\raggedleft\textbf{Related Work}}

%Goel et al. \cite{goel2019knapsack} studied the \textit{knapsack voting} mechanism for PB and show that it is incentive-compatible and welfare-maximizing under the overlap utility model. Freeman et al. \cite{freeman2021truthful} study the class of moving phantom mechanisms for incentive-compatible aggregation of votes. They show that the social welfare-maximizing mechanism is the unique Pareto-optimal mechanism in this class of mechanisms.%The ideas in their proofs, especially the one regarding how knapsack voting is related to the median of voter preferences, are used in our work to analyze the welfare-maximizing property of the Nash bargaining.

%Jain, Sornat, and Talmon \cite{jain2020} proposed a way to model project interactions in PB, including using convex and concave utility functions to model complementarities and substitutions. They consider $K$-approval voting and study the computational complexity of finding a welfare-maximizing bundle of projects.% where all the project interactions and utility functions are known \edit{to the PB designer.}
% \edit{They consider utility functions for voters which depend only on the number of  projects that they approved and get funded, and not on the costs of these projects.} %More recently, Jain, Talmon, and Bulteau \cite{jain2021partition} proposed conducting a preliminary election for aggregating the project groups before conducting the primary PB election. 
%Our sequential deliberation based method assumes that the project interactions are not known to the PB designer, and the outcome can be fractional allocations. 
%Our menu-based ballot design is similar to the model in \cite{jain2020} such that we have the PB designer gives the project groups. However, we study a different preference elicitation method and utility function from \cite{jain2020}. \edit{Our preference elicitation method collects more information regarding the preferences of the voters than $K$-approval, especially when projects have very different costs. Our utility function considers the costs of projects and is more aligned with the overlap utility model~\cite{goel2019knapsack}.}

The \textit{sequential deliberation} mechanism for social choice was proposed by Fain et al. \cite{fain2017}. They extensively analyze the mechanism in median spaces, which include median graphs and trees, and find an upper bound of the distortion of the mechanism to be 1.208. They also analyze the distortion in the \emph{budget space} (or unit simplex) and find the distortion to be $4/3$ in a special setting where each voter votes for only one project {\color{red} where each project has the same cost.} Our work extends their work in the budget space, where voters do not have this restriction on their votes and can distribute the total funds among different projects. {\color{red} Note that in our model projects do not have a pre-determined cost but agents can choose to allocate an arbitrary amount of funds to any project subject to the budget constraint along the lines of \cite{FREEMAN2021105234}.}

%Some recent works have proposed randomized voting schemes. %In Fain et al. \cite{fain2019}, voters report a pairwise comparison between randomly chosen budget proposals, 
The work most closely related to ours is by Fain et al.~\cite{fain2019}; they study a mechanism called \textit{random referee}, in which two randomly chosen voters are asked for their preferences, and another voter is randomly chosen as a referee to pick one of the two preferences. We use their technique of analyzing the pessimistic distortion of a small group of voters. However, they apply this technique where the underlying decision space is the Euclidean plane and use the underlying geometric structure to perform a grid search. In contrast, we study pessimistic distortion with Nash bargaining, which leads to a complex structure of outcomes which we capture in the form of exponentially many linear or bilinear programs. %for finding an upper bound of the distortion in obtaining our results.

Bhaskar et al. \cite{bhaskar2018truthful} study mechanisms where voters report a set of projects with utility higher than a randomly set threshold; this is somewhat orthogonal to our work where only a small set of voters need to participate. Fain et al. \cite{fain2020concentration} also analyze low-complexity randomized mechanisms for PB. However, their focus is on obtaining constant factor guarantees for higher moments of distortion instead of optimizing the constant factor, and the distortion guarantee they provide is much larger than 2.  %Our proposed sequential deliberation-based method is also a randomized voting mechanism in that it chooses bargaining agents uniformly at randomly.
%
Benade et al. \cite{benade2018} do a theoretical and empirical study of the trade-offs between different preference elicitation methods for PB. %, including knapsack votes, rankings by value or value for money, and threshold approval votes. They found that threshold approval voting is superior in maximizing the voters' unknown underlying utilities. 
Another area of focus has been fairness in PB \cite{fain2018fair,conitzer2017fair,fluschnik2019fair}.
% and finding solutions in the core \cite{fain2016core}. 
Several additional results in PB are described in the survey by Aziz et al. \cite{aziz2021participatory}.


{\raggedleft\textbf{Roadmap}}
%We describe the sequential deliberation approach for PB in Sections~\ref{sec:model_SD}-\ref{sec:exp}. Within this, 

We describe the model and preliminaries in \S~\ref{sec:model_and_prelim}; introduce a projection operation and give some technical results in \S~\ref{sec:projection_smaller_subset_voters}; characterize the outcome of the bargaining under different schemes in each round of deliberation in \S~\ref{Sec:nash_outcomes}. %{\color{blue} an overview of different bargaining schemes in \S~\ref{overview_barg_section}}, 
We derive the distortion of the relaxed Nash bargaining scheme in %after one round of deliberation in
\S~\ref{sec:distort_Nash_relaxed}. We derive the distortion under a randomised Nash bargaining scheme in \S~\ref{sec:triadic_deliberation}. Finally, we give empirical results
in \S~\ref{sec:exp} and brief concluding remarks in \S~\ref{sec:conclusion}.

%Then we discuss the second setting, i.e., the menu-based ballot design in Section~\ref{sec:MBPB}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> intro_geoff.tex <==
\section{Introduction}
More than 1500 cities around the globe have begun adopting {\it Participatory Budgeting} (PB) \cite{wainwright2003,ganuza2012}, 
a process through which residents can express their opinion
directly on a city government's use of public funds.  Citizens might, for example,
vote directly on how to allocate a budget of reserved funds between projects like
street repairs, library renovations, or public art installations.  PB has been shown to promote
government transparency, citizen engagement, and good governance \cite{wampler2007}.

PB implementations have used a wide variety of voting mechanisms to elicit preferred budgets from citizens 
\XXX{cite many examples of voting mechanisms?}, yet no matter the mechanism,
policymakers must transform a list of votes on a budget into a real-world allocation of funds.
\XXX{check this next line}
Furthermore, even though there may \XXX{is? sometimes is?} be an ``optimal'' allocation (under natural notions
of social welfare),
this allocation may be intractable to compute or difficult to reliably estimate if turnout is low.
Our topic of study in this work is the {\it distortion} that aggregation mechanisms introduce
between the theoretically ``optimal'' allocation and the allocation output by a mechanism.

In particular, we focus on a process known as {\it sequential deliberation} \cite{fain2017,fishkin2018democracy},
a mechanism for collective decision-making (in contexts where citizens can debate directly)
 that we adapt into an aggregation mechanism for PB.
In each round of sequential deliberation,
two randomly-selected voters debate to decide on a compromise, which becomes the ``disagreement point''
for the next round.  If the voters in a round fail to reach a compromise, their choice defaults to the disagreement
point of the previous round; as such,
the disagreement point, in essence, captures an aggregate preference of the deliberators of previous rounds.
To extend this process to PB (where a ``deliberation'' must be between static votes, not living voters),
we propose and analyze several \XXX{several? one? two?} classes of ``bargaining'' mechanisms for algorithmically aggregating two random budget votes
and a disagreement point into a new disagreement point (and let the disagreement point of the first round be a third, random vote).

We specifically give theoretical guarantees on the worst-case performance of this process after one round of deliberation.
\XXX{be more specific?} We find that even one round of deliberation gives a substantial improvement over many natural classes
of simpler mechanisms.  We also apply our mechanism to real-world PB votes, and show empirically that sequential deliberation
converges quickly to a good \XXX{some other word for good?} outcome.

One important feature of sequential deliberation is that the outcome
is guaranteed to be either the preference of an individual or of a pair of individuals;
this means that the outcome will always account for complex interactions between different projects (such as substitutability and complementarity \cite{jain2020, jain2021partition}).

%\XXX{move to our results section}
% We define these terms precisely and show that our proposed mechanism naturally accommodates these complex preferences in the Appendix \S \ref{sec:TD_project_interaction}. 
%}



Sequential deliberation as a mechanism may be of independent interest to policymakers implementing PB.  A few rounds of
simulated deliberation could, for example, allow policymakers to estimate with a small sample of voters the result of a possible
PB vote; this could be particularly important in scenarios where turnout is low
or a PB ballot must be simplified before deployment. \XXX{citations}

\subsection{Our Contributions}

To measure the quality of an aggregation mechanism,
we follow Ashelevich et al. \cite{anshelevich2017randomized} and study
the \textit{distortion} of a mechanism, which measures the \emph{social cost}
of the output budget relative to a budget that minimizes social cost.
We specifically study the case where the social cost is the sum of the $\ell_1$ distances
between an output budget and the votes of each voter.

We show first that natural mechanisms, such as randomized dictator, and even mechanisms where two random votes deliberate 
\textit{without} a disagreement point cannot have a distortion less than $2$.

In contrast, we show that the use of a disagreement point
enables mechanisms that are guaranteed to have distortion substantially below $2$.
Specifically, we show first that all bargaining mechanisms in a class of \emph{median margaining schemes} achieve distortion
of at most $1.83$ after just one round of deliberation.  Furthermore, we also give a \emph{randomized Nash bargaining scheme}
that achieves distortion of at most $1.66$ after one round.

Our main technical tool is our analysis of \emph{pessimistic distortion} (first proposed in Fain et al. \cite{fain2019}),
which upper-bounds the distortion.
Instead of one ``optimal'' budget, the pessimistic distortion measures distortion against many allocations, 
each of which is tailored to a small group of voters. \XXX{is it really necessary to explicitly define pessimistic distortion here?}
We then transform the problem of computing the pessimistic distortion into a large set of linear programs (for median bargaining schemes)
or bilinear programs (for randomized Nash bargaining).  \XXX{is this true?} We find and exploit symmetries in the structure of these programs
to reduce their number, and then \XXX{mechanically?} solve them all to bound the pessemistic distortion.


Finally, we evaluate our proposed mechanism \XXX{which bargaining scheme? randomized nash? median?}
on the empirical results of four real PB elections.
In each election, the expected distortion after just two rounds of sequential deliberation is less than $1.30$.
Furthermore, the variance of the output allocations converges to a small value \XXX{I don't know how to frame this, but something other than 
"a small value" would be good} after three rounds of deliberation. %This validates our approach on real-world datasets. % what elections? % should we include fast convergence here?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

We describe the model and preliminaries in \S~\ref{sec:model_and_prelim}, characterize the outcome of the bargaining in each round of deliberation in \S~\ref{Sec:nash_outcomes}, and derive the distortion of the relaxed Nash bargaining scheme after one round of deliberation in \S~\ref{sec:distort_Nash_relaxed}. 
We derive the distortion under a randomised Nash bargaining scheme in \S~\ref{sec:triadic_deliberation}. Finally, we give empirical results
in \S~\ref{sec:exp}.

%Then we discuss the second setting, i.e., the menu-based ballot design in Section~\ref{sec:MBPB}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> menu_based_allocation.tex <==
\section{ Menu-based Ballot Design}
\label{sec:MBPB}
The model and notation of this section are different from the previous sections; however, all the new notation is defined explicitly.

\edit{Recall that in the menu-based ballot design, the PB designer gives a partition of projects into groups. The voters allocate funds to different groups as in knapsack voting and do approval voting for projects within a group, as explained in the introduction. 
%Our sequential deliberation-based approach to PB works under some assumptions which we attempt to relax in the menu-based ballot design. 
This proposal works like a traditional PB election in which every voter casts her vote, as opposed to a random sample of voters being involved in the decision-making process in sequential deliberation. This approach can handle both fractional and non-fractional allocations to projects, however, we consider only the case of non-fractional allocations in this paper. We have the following differences in the model in comparison to the sequential deliberation-based setting:

\begin{enumerate}[leftmargin=*]

\item The project interactions are given by the ballot designer in the form of a partition of the projects into groups
\item \emph{Voter need not agree on interactions between projects within a group.} Our menu-based ballot design and the associated utility function can handle more complex substitution project interactions than just perfect substitutes.
%\item \emph{All voters agree on the project interactions.} 
For projects within a group, voters have the option of approving only a subset of the projects. This indicates which projects from within the group they like. If a voter consider these projects to be substitutes, they may allocate a smaller amount of funding to this group in their knapsack allocation than is required to fund all their approved projects in the group. %This indicates that they are indifferent to which of their approved projects are funded, but they are \emph{satiated} at a certain amount of funding for the group.
\end{enumerate}

We further illustrate the model with an example.

\textbf{Example 6.1:} Consider a simple instance of a PB election with a total budget of $ \$4M$ and the following six projects:
\begin{enumerate}[leftmargin=*]
\item Increase the support to homelessness prevention, outreach, and shelter programs. \hfill \emph{Cost: \$ 2M}.
\item A technology upgrade in the police department. \hfill  \emph{Cost: \$ 1M.} 
\item Install street lights in some crime-prone areas. \hfill  \emph{ Cost: \$ 1M.}
\item Hire $10$ additional police officers in the city. \hfill  \emph{ Cost: \$ 2M.}
\item Widen the car lane on street X. \hfill  \emph{Cost: \$ 1M.}
\item Construct a bike lane on street X. \hfill  \emph{ Cost: \$ 1M.} 
\end{enumerate}

The PB designer will categorize the projects as: 
\begin{itemize}[leftmargin=*]
\item \emph{Group A} [Homelessness Prevention]: Project (1).
\item \emph{Group B} [Public Safety]: Projects (2), (3), and (4).
\item \emph{Group C} [Road Construction]: Projects (5) and (6).
\end{itemize}

The projects in Group C are contradictory since projects (5) and (6) cannot be done together due to a natural space constraint near street X. Further, some voters may think that the projects in Group B are substitutes for each other. More importantly, in our menu-based ballot design, the voters need not agree whether the projects in Group B are substitutes or not. Project (1) is independent.

Consider voter $i$ who believes that the projects in Group B are not substitutes and would like that projects (3) and (4) be funded. Voter $i$ would allocate $\$3M$ to the Group B in the knapsack vote and approve projects (3) and (4) within it. Another voter $i'$ believes that the projects in Group B are substitutes, however she does not like project (3). Further, she believes that spending a total of $\$2M$ on public safety related enhancements is the right thing to do in this PB election. She would allocate $\$2M$ to Group B and approve projects (2) and (4). In other words, voter $i'$ has a \emph{subadditive} utility in projects (2) and (4) which gets saturated at $\$2M.$}


%In the ballot design proposed in this section, we consider the preference elicitation model of knapsack votes across groups and approval votes within each group. The groups, designed by the ballot designer, contain projects with interacting utilities or having a common theme. For example, the groups can be a broad classification of the projects (e.g. police reforms, healthcare, etc.). The projects in the groups can be specific actions with well-defined costs. 

\subsection{Formal model}
Let the set of projects be $Q$, which is partitioned into $q$ groups $Z_1, \ldots, Z_q,$ by the PB designer such that $Z_1 \cup Z_2\ldots \cup Z_q = Q.$ The vote of voter $i$ is denoted by $v^i$, where $v^i_c$ for group $c$ is the tuple $(f^i_c, S^i_c),$ such that $S_c^i \subseteq Z_c,$ are the projects that voter $i$ approves in group $c,$  $f^i_c \geq 0$ is the amount of funds that voter $i$ allocates to group $c$ in the knapsack vote over groups, and $\sum_{c=1}^q f^i_c = B$ where $B$ is the total budget. \edit{The cost of  project $p$ is $C(p).$} We now give the utility function for this setting, which is a natural modification of the overlap utility function~\cite{goel2019knapsack}.
% and then give results corresponding to the computational tractability of finding a social welfare-maximizing budget.

For an outcome which fund projects in the set $P \subseteq Q$, the utility for a voter $i$ with vote $v^i : v^i_c = (f^i_c, S^i_c)$ is
\begin{equation}
 u_i(P) = \sum_{c=1}^q ~\min \left(f_c^i, \sum_{p \in \{P \cap S_c^i\}} C(p) \right). \label{eq:utility}
\end{equation}
This  utility function is reminiscent of the Leontief-free (LF) utility function defined by Garg, Mehta, and Vazirani in \cite{garg2018substitution} in the context of a private goods economy to capture the subadditivity of the joint utility of a bundle of goods that are substitutes. They refer to this utility structure also as \emph{substitution with satiation.} One key difference of \eqref{eq:utility} with LF is that  in \eqref{eq:utility}, the amount of funding at which the utility saturates is related for different groups via the knapsack budget constraints, whereas it is independent in LF. %Another difference is that \cite{garg2018substitution} considered \emph{fractional} quantities of consumption of different goods for a consumer, whereas we primarily study non-fractional funding of projects.}% and each good in a group con potentially have a different utility per-unit.}
% for a consumer.

\edit{Note that the ballot design of~\cite{jain2020} also models complementary projects, in addition to substitutes, while our model does not. This simplification  enables us to adopt a more natural utility function which depends on the costs of projects that are funded. Whereas, their utility function depends only on the number (and not the cost) of projects that are common between a voter's vote and the outcome of the preference aggregation algorithm. Further, this simplification makes our model amenable to studying strategic behavior of voters. Additionally, for completeness we show that some results regarding computational complexity from~\cite{jain2020} hold for our model as well. }
 

\subsection{Incentive Compatibility}
In the following lemma, we show an incentive-compatibility result for our model in a special case.
\begin{lemma} \label{lem:sp}
\edit{For unit-cost projects,} when preference aggregation is done to maximize social welfare, and at most one project from a group can be funded, the proposed voting mechanism is strategy-proof.
\end{lemma}
\begin{proof}
When at most one project from a group can be funded\edit{\footnote{\edit{This is the case, for example, when the projects in a group are contradictory. It is also the case when projects in a group are perfect substitutes for all voters.}}}, for social welfare-maximizing preference aggregation, it can only be the project with the most approvals in that group.

There can be three types of deviations from the truthful vote of a voter. First is: not approving a project $p$ which they like. This deviation can cause only one change to the outcome, if at all. That is: project $p$, which would otherwise get funded, does not get funded and instead of $p,$ another project $q$ gets funded. This deviation does not change the utility of the voter if they like project $q$ and reduces it if they do not like project $q.$ The second type of deviation is: approving a project $r$ which they do not like. This deviation can change the outcome in only one way. That is: project $r$, which would otherwise not get funded, gets funded. Since the voter does not like project $r$, this deviation cannot increase their utility.

The third deviation is in the knapsack vote over groups. Note that in this special case where at most one project from a group can be funded, every voter allocates at most one unit of funds to a group in their truthful knapsack allocation vote. Deviating by allocating funds to a group that is not funded in their truthful vote cannot increase the utility, since it can only increase the allocation to a project that they do not like. %Further, increasing the funding to a group that they already fund in their truthful vote can also not increase their utility because only one project from a category can be funded. 
\qedhere


% A deviation from the truthful strategy in allotting funds to groups (knapsack vote over groups) can never increase the utility of a voter since the voter does not get any utility from a group they would not fund in their truthful vote in our utility model (which is an adaptation of the overlap utility model). %This follows from the strategy-proofness result for the knapsack voting scheme \cite{goel2019knapsack}.  

%For a group to which the voter allocates a unit of fund in her truthful vote, approving an extra project $j$ can only increase the chances of funding of project $j$. This does not increase the overlap utility of the voter since that project is not approved in her truthful vote. Deviating from the truthful vote by not approving a project $j'$ can make only one type of change to the final allocation. This is the case when the deviation causes project $p$ to be not funded and some other project $q$ to be funded instead of it. This will give a utility change of $0$ if the voter approves $q$ and $-1$ if the voter does not approve $q$. The argument also holds for multiple simultaneous deviations in project approvals since it can be analyzed in steps of one deviation at a time. No step can strictly increase the overlap utility of the voter.
\end{proof}
%Lemma~\ref{lem:sp} holds, for example, if the projects in a group are either perfect substitutes or are contradictions. %We give a proof for the non-fractional allocation case in Appendix~\ref{proof_sp}. The result also holds for the fractional allocation case by a similar argument. 

However, as we show in Appendix~\ref{not-IC}, strategy-proofness does not hold for our model when more than one project from a group can be funded. %in general for the social welfare-maximizing preference aggregation. %This is true for both the greedy and the maximum welfare preference aggregation schemes.
\begin{comment}
Due to the submodularity of social welfare (Lemma~\ref{lem:submodular}), it is possible to have the following scenario. If two projects were to be funded from group $c$, then those would be projects $p_1$ and $p_2$, and if three projects were to be funded from group $c$ then those would be projects $p_3, p_4,$ and $p_5$. Consider voter $i$ whose truthful vote for group $c$ is as follows: allocate $f_c^i = 3$ units of funds and approve projects $p_1, p_2,$ and $p_3$. Under some vote profiles, voter $i$ has an incentive to strategically not approve project $p_3,$ and report $f_c^i = 2.$ This deviation can cause the optimal funding to group $c$ to reduce from $3$ units to $2$ units. This results in the allocation of funds to projects $p_1$ and $p_2$ instead of projects $p_3, p_4,$ and $p_5,$ thereby increasing voter $i$'s utility by $1$ unit.
\end{comment}

%\textbf{Lack of $\alpha$-additive incentive compatibility:} A similar example can show that $\alpha$-additive incentive compatibility also doesn't hold for the welfare-maximizing preference aggregation. In this case consider $2k+1$  projects $p_1, p_2,\ldots, p_k,$ $ q_1, q_2,\ldots, q_k, r.$ in the same group. Let if $k$ of these are to be funded then $p_1,\ldots, p_k$ are funded and if $k+1$ are to be funded then  $q_1, q_2,\ldots, q_k, r$ are funded. Consider a voter who truthfully approves $p_1,\ldots, p_k, r.$ This voter has an incentive to approve only $p_1,\ldots, p_k$ and force only $k$ projects to be funded from this group. Here this voter gains an incentive of $k$ units due to strategic behavior.

%Even when we allow at most two projects from a group to be funded, there is opportunity for strategic behavior. For example, consider that voter $i$ likes projects $p_1$ and $p_2$ from group $A$ and only project $p_3$ from group $B$. Further, voter $i$ knows that $p_2$ is unlikely to be funded. Then she has an incentive to not approve $p_2$ and rather approve a project $p_4$ which strengthens the chances of $p_3$ being funded. This can happen when $p_3$ and $p_4$ are complements and the complement pair $(p_5, p_6)$ is a substitute for the pair $(p_3, p_4).$
\subsection{Computational Complexity}
% One typical objective is to maximize the social welfare.%, $U(P) = \sum_{i \in [n]} u_i(P)$.
Observe that the social welfare function $U(P)$, which the sum of $u_i(P)$ for all voters $i \in [n],$ satisfies the following result.
\begin{lemma}\label{lem:submodular}
$U(P)$ is a submodular function over the subsets of $Q$.
\end{lemma}
%The proof is simple and is in Appendix~\ref{proof_submodular}.
\begin{proof}
Notice that the utility obtained from funding a project can only decrease if other projects from the same group are already funded. This is because of the subadditive nature of the utility function $u_i(P)$. The social welfare is therefore a sum of $n$ submodular functions, one for each voter, and is itself submodular.
\end{proof} 

%\begin{corollary}
%The greedy algorithm for preference aggregation is $(1-\frac{1}{e})$-competitive for maximizing the social welfare.
%\end{corollary}

We have the following result for the computational complexity of maximizing the social welfare under non-fractional allocations.
\begin{lemma} \label{lem:nphard}
Social welfare maximization is \emph{NP-hard.}
\end{lemma}
%The result is obtained via a reduction from the maximum set coverage problem. The proof is in Appendix~\ref{proof_nphard}.
\begin{proof}
The result is obtained via a reduction from the maximum set coverage problem. Consider the case where each project is unit-cost and each vote $v^i_c$ has $f^i_c$ equal to either $0$ or $1$ for all groups $c \in [q].$ 
%Recall that there are $n$ voters and $q$ groups of projects. 
We make $B$ copies of each voter, each copy corresponding to a group they funded in their vote. These $nB$ entities (or voter-group pairs) form the elements of the set $T$, which is to be covered maximally. Each project corresponds to a subset of $T$, and there are $m$ such subsets. Specifically, the subset of $T$ corresponding to project $j$ in group $c$ contains the voter-group pairs for those voters who funded group $c$ and approved project $j$. %Denote these subsets by $P_k$ for $k \in [m]$. 
Out of these $m$ subsets of $T$, $B$ are to be chosen with the objective of maximizing the coverage of $T$. This problem, which is known to be NP-hard, is now equivalent to maximizing the social welfare in our model.
\end{proof}

In Appendix~\ref{efficient-computation}, we show that social welfare maximization can be done efficiently if the maximum size of a group is not large. Specifically, we give a dynamic programming based algorithm for preference aggregation, which runs in time linear in $q$ and $B$ and exponential in the maximum size of a group. In the special case where all projects are of equal cost, this algorithm is fixed-parameter tractable (FPT).
\begin{comment}
We now show that social welfare maximization can be done efficiently if the maximum size of a group is not large. %This result is inspired from~\cite{jain2020}, who obtain it for $K-$approval voting scheme and a different class of utility functions in which project groups could be substitutes or complements.
%\begin{lemma} \label{lem:fpt}
%Social welfare maximization is \emph{FPT} with respect to the maximum size of a group.
%\end{lemma}
%The proof is given in Appendix~\ref{proof_fpt} via dynamic programming. 
%\begin{proof}
 We give an algorithm for preference aggregation, which runs in time linear in $q$ and $B$ and exponential in $s$: the maximum size of a group. %We make use of the fact that the utilities are additive across group of projects.
For each possible fund allocation to group $c$ ranging from $0$ to $\min(B,\sum_{p \in z_c} C(p)),$ compute the total utility of the \emph{best subset} of $z_c$. Here, this best subset is the one that maximizes the total utility from projects of group $c$. This best subset and  total utility can be computed for all possible values of funds allocated to group $c$ in time $O(2^{|z_c|} |z_c|)$ by checking each subset of $z_c$. Denote the total utility obtained on allocating funds $b$ to group $c$ by $h_c(b).$ 

Since the total utility is additive across groups, we now have a problem of splitting of budget optimally between the $q$ groups. That is, social welfare maximization is equivalent to the following:
\begin{align}
\text{Maximize} ~~ \sum_{c=1}^q h_c(b_c) \ \ \ \text{subject to} ~~ \sum_{c=1}^q b_c = B. \label{eq:optimization}
\end{align}
%Note that $h_c(b_c)$ is non-decreasing in $b_c$ for all groups $c \in [q].$ 
Denote the optimal allocation of budget $B$, subject to the availability of only groups in set $G,$ by $U_{G}(B)$. Under this notation, the optimal value of problem~\eqref{eq:optimization} is $U_{[q]}(B).$ % and the optimal allocation of budgets to the groups for total budget $B$ by $b^B_j$ for all groups $j \in [q].$ 
To solve this problem, we run a dynamic programming \cite{bellman1966dynamic} algorithm which solves:
$$ U_{[q]}(B)  = \max_{ b \in [B]} ~\{  U_{[\left \lfloor{q/2}\right \rfloor ]} (b) +  U_{[q]\backslash [\left \lfloor{q/2}\right \rfloor ]} (B-b)  \}.$$  
Storing the intermediate outputs allows finding the set of projects which achieve $U_{[q]}(B).$ See that the given algorithm runs in $O(qB)$ time and it fills a table with $qB$ entries.\edit{\footnote{\edit{This algorithm is reminiscent of the dynamic programming-based pseudo-polynomial time for the knapsack problem \cite{bellman1966dynamic}. Since the cost of projects is typically given only up to a precision $\textsc{Pre}$ of $1/1000 -$th part of $B,$ we need not have a complexity of $O(qB),$ but only  of $O(q \cdot B/ \textsc{Pre}).$ For example, in an election with a $\$ 5M$ budget,  the costs of projects may be defined to a precision of $\$ 10K.$ In this case, we need to store $\frac{\$ 5M}{\$10K} = 500$ entries for each group of projects in our algorithm.   }}}
%\end{proof}
\end{comment}

\begin{comment}
We now discuss fractional allocations in our model, which may be useful in PB elections where projects do not have a fixed cost or can be completed to different degrees, depending on how much funds are allocated to them.

\subsection{Fractional Allocations}
Under fractional allocation $x$, the overlap utility for voter $i$ is:
\begin{equation}
 u_i(x) = \sum_{c =1}^q ~\min\left(f_c^i, \sum_{j \in S^i_c} x_j\right).
\end{equation}  
The utility is additive across groups. Within a group $c$, the voter $i$ gets utility from allocation to their approved project, but only up to $f_c^i$.  We now show that efficient preference aggregation is possible by solving a convex program.

The problem of preference aggregation can be given as :
\begin{align*}
&\text{Maximize~~~~~} G(x) \\
&\text{Subject to~~~} \sum_{j \in [m]} x_j \leq B,
\end{align*}
for some function $G(x)$ of the budget $x$. Typical choices of $G(x)$ are the social welfare: $U(x) = \sum_{i \in [n]} u_i(x)$, the minimum welfare: $U_{\min}(x) = \min_{i\in[n]} u_i(x)$, and the Nash welfare: $U_{NW}(x) = \sum_{i\in[n]} \log(u_i(x)).$ 
%\begin{align}
%&\text{Maximize~~~~~} \sum_{i \in [n]} u_i(x) \\
%&\text{Subject to~~~} \sum_{j \in [m]} x_j \leq B.
%\end{align}
%Similarly, the Nash welfare-maximizing preference aggregation problem is:
%\begin{align}
%&\text{Maximize~~~~~} \sum_{i \in [n]} \log(u_i(x))  \\
%&\text{Subject to~~~} \sum_{j \in [m]} x_j \leq B.
%\end{align}
%The max-min problem is:
%\begin{align}
%&\text{Maximize~~~~~} \min_{i \in [n]} u_i(x)  \\
%&\text{Subject to~~~} \sum_{j \in [m]} x_j \leq B.
%\end{align} 
From the definition of $ u_i(x)$, is is clear that it is a concave function of $x.$ Similarly, $\log(u_i(x))$ is a concave function of $x$. Since the sum and minimum of concave functions are concave, all the three problems defined above are maximization of concave functions. They can therefore be solved in polynomial time~\cite{boyd2004convex}.
\end{comment}



==> preliminaries_geoff.tex <==
\section{Preliminaries}
\label{sec:model_and_prelim}
\subsection{Budgets and Distortion}


A \emph{budget} allocates funds between $m$ projects.  We normalize the total amount of funds to $1$, and assume
that no project has a fixed cost; that is, each project can be allocated any amount of money.

\XXX{why not just call it a simplex?}
\begin{definition}[Budget Simplex]
The {\it Budget Simplex} $\mathbb{B}$ is the set of all valid budgets, $\lbrace b \in \mathbb{R}_{\geq 0}^m \vert ~\Sum_{i=1}^m b_i = 1\rbrace$.  
\end{definition}

\XXX{why doesn't vote profile get a definition box?}
Each voter $i$ produces a preferred budget vote $v_i\in \mathbb{B}$.  
A collection of votes from each voter is a \emph{vote profile} $P=(v_1,...,v_n)$.

\begin{definition}[Cost]
In our model, the \emph{cost} of a budget $b$ to a user with preferred budget $v$ is the $\ell_1$ distance
between the two budgets, $d(b, v)=\Sum_i \vert b_i-v_i\vert$.  The \emph{social cost} of a budget $b$ with respect to a vote profile
is the sum of the costs
of $b$ with regard to each voter's preferred budget.
\end{definition}

An equivalent view of the cost of a budget is a voter's \textit{overlap utility}.

\begin{definition}[Overlap Utility]
\label{def:ou} The \textit{Overlap Utility} of a budget $b$ with respect to a vote $a$ is $u(a,b) = \Sum_{j=1}^{m} \min(a_j,b_j).$
\end{definition}

\begin{lemma}
\label{disutility}
For any two budgets $a,b \in \mathbb{B}$, $d(a,b) = 2 - 2u(a,b)$.
\end{lemma}
Appendix~\ref{} gives a proof.

Note that overlap utility is symmetric ($u(a,b) = u(b,a)$), and that $u(a,a)=1$ for all $a \in \mathbb{B}$.


\XXX{Put definition of distortion here (just add in all of previous section 2.2, although I'm sure the latter half of the section
can be cut in length by 1/2 without cutting content.

Then the deliberation model.

Then, in the next subsection, define this incremental allocation thing.

}

==> project_substitution.tex <==
\label{sec:TD}
In this section, we analyze the outcome of triadic deliberation. We start with a motivating example.

\edit{\textbf{Example 3.1.}} Suppose that there are two voters $i$ and $i'$ and two projects that are \edit{perfect} substitutes for each other, and that $i$ votes for budget $\langle 1, 0 \rangle$ and $i'$ votes for budget $\langle 0, 1 \rangle$. If the outcome of the PB is $\langle 0.5, 0.5 \rangle$ (which can be a result of social welfare-maximizing aggregation with proportional tie-breaking), then the \edit{overlap} utility of each voter is $0.5$. However, if the outcome is $\langle 1, 0 \rangle$, then the \edit{overlap} utility of each voter is $1$ since the projects are \edit{perfect} substitutes. Note that even though the former outcome appears fairer to someone who does not know the project interactions, it is not optimal. This example illustrates the need to take project interaction into account while designing a voting scheme for PB.

%We model complementarity and substitutions as follows. 
%\edit{Mathematically, we model project interactions as follows:} if projects in group $q$ are perfect complements of each other, then the utility that voters can derive from each project in $q$ is the minimum funding of any project in $q$. For example, if the software and hardware projects are funded $0.2$ and $0.5,$ they can only use $0.2$ each, and the excess funding of $0.3$ for the hardware project is wasted. If the projects in group $r$ are \edit{perfect} substitutes, then the utility that voters can derive from group $r$ is the maximum funding of a project in $r$. For example, if two companies are paid $0.2$ and $0.5$ to do the same work, only $0.5$ will be used, and $0.2$ is wasted.

%We now provide a formal model. 
Let $m_c$ denote the number of groups of \emph{perfect complementary} projects, $m_s$ denote the number of groups of \emph{\edit{perfect} substitute} projects, and $m_r$ denote the number of \emph{regular} projects. Let $s(q)$ denote the number of projects in group $q$. For groups of perfect complementary and \edit{perfect} substitute projects, $s(q) \ge 2$ and for regular projects $s(q) = 1.$ The total number of projects is $m = \left( \sum_{q=1}^{m_c + m_s} s(q) \right)+ m_r$.
For simplicity, %assume that project groups are arranged in the order such that complementary projects come first, followed by \edit{perfect} substitute projects, and then regular projects. 
project groups are arranged such that groups $1, \ldots, m_c$ are perfect complementary, groups $m_c+1, \ldots, m_c+m_s$ are \edit{perfect} substitutes, and $m_c+m_s+1, \ldots, m_c+m_s+m_r$ are regular projects.
%Let $u(x, y)$ denote the \emph{utility function} of budgets $x$ and $y$. Define $u(x, y) = u'(f(x), f(y))$ where $u'(p, q) = \sum_i \min(p_i, q_i)$ is the overlap utility between $p$ and $q$.

Let $f(b)$ be the \emph{efficiency function} which captures how much budget $b$ respects the project interactions. Specifically, $f(b)$ takes a budget $b \in \mathbb{R}^m$ and outputs a vector in $\mathbb{R}^{m_c+m_s+m_r}$, where
\begin{align*}
f(b)_i = \begin{cases}
s(i) \min(b_j ~|~ j \in \mbox{group }i) &\mbox{if } i \in [1, m_c], \\ 
\max(b_j ~|~ j \in \mbox{group }i) & \mbox{if } i \in [m_c+1, m_c+m_s], \\
(b_j ~|~ j \in \mbox{group }i) & \mbox{otherwise.} %\mbox{if } i \in [m_c+m_s+1, m_c+m_s+m_n]
\end{cases}
\end{align*}
For a group of perfect complementary projects, the corresponding output element is the bottle-neck allocation in the group, multiplied by the number of projects in the group. For a group of \edit{perfect} substitute projects, the corresponding output element is the largest allocation in that group. For regular projects, the corresponding output elements are the same as the allocation to the project.
%For example, suppose that $m_c = 1$, $m_s = 1$, and $m_n = 1$. If $b = \langle .4, .3, .2, .0, .1 \rangle$, then $f(b) = \langle 2\min(.4, .3), \max(.2, .0), .1 \rangle = \langle .6, .2, .1 \rangle$.

We now define the overlap utility between a pair of budgets.
\begin{definition} \label{def:ou}
The \textbf{overlap utility} of budgets $x$ and $y$ is given by $u(x, y) = \sum\limits_{i=1}^{m_c+m_s+m_r} \min(f(x)_i, f(y)_i)$.
\end{definition}

In other words, the overlap utility of budgets $x$ and $y$ captures how much is common between the two budgets, taking project interactions into consideration. %For example, if there are two projects on the ballot and they are \edit{perfect} substitutes, then budget $\langle 0,1 \rangle$ and $\langle 1,0 \rangle$ have a overlap of $1$. However, if the projects are independent, then budgets $\langle 0,1 \rangle$ and $\langle 1,0 \rangle$ have a overlap of $0$.
 \edit{Note that the overlap utility of an agent with a preferred budget $a$, from a budget $b$ is $u(a,b).$}
%The utility that voter $i$ gets from a budget $x$ 

%An outcome of $\Nash(x, y, a)$, the \emph{Nash bargaining} between two voters with preferred budgets $x$ and $y$ and the disagreement point $a$, is a budget $z$ that maximizes the \emph{Nash product} $(u(x, z) - u(x, a)) \times (u(y, z) - u(y, a))$, subject to individual rationality $u(x, z) \geq u(x, a)$ and $u(y, z) \geq u(y, a)$, and in case of a tie maximizes $u(a, z)$.

%We define a natural modification of the overlap utility function to account for the efficiency of allocations, as captured by function $f(b).$ Define the  between $x$ and $y$ in this section to be $u(f(x), f(y))$. {\color{red}{TODO}}  This definition takes complementarity and substitution into account. For example, suppose that there are two projects that are substitutes for each other. If an voter's preferred budget is $\langle 0, 1 \rangle$, and the outcome of the PB is $\langle 1, 0 \rangle$, then the utility that they get is 1, because $u(f(\langle 0, 1 \rangle), f(\langle 1, 0 \rangle)) = u(\langle 1 \rangle, \langle 1 \rangle) = 1$.

\edit{In the following definition we formally state the requirements for a budget to be consistent with the project interactions.}
\begin{definition}
A budget $b$ \textbf{respects the project interactions} iff projects in each perfect complementary group are funded equally, and at most one project in each \edit{perfect} substitute group is funded \edit{at all.}
\end{definition}

The following lemma states that the efficiency function sums to $1$ iff the budget doesn't make inefficient allocations.

\begin{lemma}
\label{cs_sum}
Budget $b$ respects the project interactions iff the efficiency function $f(b)$ satisfies $\sum_i f(b)_i = 1$. Otherwise, $\sum_i f(b)_i < 1.$
\end{lemma}
The proof of Lemma~\ref{cs_sum} is simple and is in Appendix~\ref{cs_sum_proof}.

%The following lemma implies that the outcome of triadic deliberation respects the project interactions.
\begin{theorem}
\label{cs_main}
%Let $x$, $y$, and $a$ be budgets. 
If budget $x$ or $y$ respects the project interactions, then for any budget $a \in \mathbb{B},$ $\Nash(x, y, a)$ respects the project interactions.
\end{theorem}
%
\begin{proof}
Let $z$ be an outcome from $\Nash(x, y, a)$.
Assume w.l.o.g. that $x$ respects the project interactions, and suppose that $z$ does not. By Lemma~\ref{cs_sum},
$\sum_i f(x)_i = 1$ and $\sum_i f(z)_i < 1$.
Thus, there exists some $k$ where $f(x)_k > f(z)_k$.
By Lemma~\ref{cs_new_b} in Appendix~\ref{app:cs_new_b},
there exists a budget $z'$ \edit{which respects the project interactions and} $f(z')_i \geq f(z)_i$ for all $i$ and $f(z')_k > f(z)_k$. The overlap utility functions satisfy:
%
\begin{align*}
&u(x, z') = \sum_i \min( f(x)_i, f(z')_i ) > \sum_i \min( f(x)_i, f(z)_i ) = u(x, z), \\
&u(y, z') = \sum_i \min( f(y)_i, f(z')_i ) \geq \sum_i \min( f(y)_i, f(z)_i ) = u(y, z).
\end{align*}
%Since u'(x, z') > u'(x,z) and u'(y,z') \geq u'(y,z), z is not an outcome from a Pareto-efficient bargaining, a contradiction.
%Since $u(f(x), f(z')) > u(f(x), f(z)),$ $u(f(y), f(z')) \geq u(f(y), f(z))$, 
This implies that the Nash product of \edit{overlap utilities with} $z'$ is higher than that with $z$, a contradiction. 
\end{proof}
%The proof is in Appendix~\ref{proof_cs_main}.

Theorem~\ref{cs_main} implies that if every voter has a preferred budget that respects the project interactions, then the outcome of the sequential deliberation mechanism will always respect the project interactions, no matter how many rounds it runs. Another important implication of this result is that if sequential deliberation works \edit{well} for PB without project interactions, then it will also work \edit{well} for PB with project interactions. %\sukolsak{I'm not sure anymore if this theorem is that useful.}
 
%Note that Theorem~\ref{cs_main} holds not only with the Nash bargaining, but also with any bargaining solution that is Pareto-efficient, such as the Kalai-Smorodinsky solution \cite{kalai1975} or the egalitarian solution \cite{kalai1977}. Although we use the Nash product in the proof, the last paragraph in the proof is simply the definition of Pareto efficiency.

Now we characterize the total utility of the three voters, two involved in the bargaining and one whose preferred budget is chosen as the disagreement point, under the Nash bargaining solution. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

